Federated Few-Shot Learning with Adversarial Learning

We are interested in developing a unified machine learning model over many mobile devices for practical learning tasks, where each device only has very few training data. This is a commonly encountered situation in mobile computing scenarios, where data is scarce and distributed while the tasks are distinct. In this paper, we propose a federated few-shot learning (FedFSL) framework to learn a few-shot classification model that can classify unseen data classes with only a few labeled samples. With the federated learning strategy, FedFSL can utilize many data sources while keeping data privacy and communication efficiency. There are two technical challenges: 1) directly using the existing federated learning approach may lead to misaligned decision boundaries produced by client models, and 2) constraining the decision boundaries to be similar over clients would overfit to training tasks but not adapt well to unseen tasks. To address these issues, we propose to regularize local updates by minimizing the divergence of client models. We also formulate the training in an adversarial fashion and optimize the client models to produce a discriminative feature space that can better represent unseen data samples. We demonstrate the intuitions and conduct experiments to show our approaches outperform baselines by more than 10% in learning vision tasks and 5% in language tasks.

==> sections/symbol.tex <==
\begin{table}[htb]
\caption{Frequently used notations.}
\vspace{-3pt}
\begin{tabular}{c|l}
\toprule  
\textbf{Notation}  & \textbf{Description}  \\ \toprule
$\mathcal{T}$ & an episode, i.e., a sampled task with support and query set  \\
$\mathcal{T}^{(s)}$ & the support set of an episode \\
$\mathcal{T}^{(q)}$ & the query set of an episode \\
$P$-shot & number of training samples in support set of a sampled task \\ 
$N$-way & number of classes in support/query set of a sampled task \\
$Q$-query & number of samples in query set of a novel task \\ 
$K$ & number of clients \\ 
$C$ & fraction of clients updated in parallel \\
% $p(\mathcal{T})$ & the task distribution \\ 
% $\alpha$ &  Startup time of a single operation of gradients aggregation. \\
% $\beta$ & Transmission and aggregation time per gradient. \\
$w$ & meta-learning model, $w=\Tteq$ \\
$f_{w}$ & FSL model parameterized with $w$   \\
$F_{w}$ & task loss function induced by model $f_{w}$ \\
$\Theta$ & feature generator (FE) of a meta-learning model \\
$\theta$ & classifier (CLF) of a meta-learning model \\
$f_{\Theta,\theta}$ & FSL model parameterized with FE and CLF   \\
$\alpha$ & learning rate \\
% $L$ & The number of learnable layers (or tensors) of a deep model. \\
% titer & Time of an iteration. \\
% tf & Time of the forward pass in each iteration. \\
% tb & Time of the backward pass in each iteration. \\
% tu &  Time of the model update in each iteration. \\
% t1 & Time of the gradient calculation of layer l in each iteration. \\
% $\tau$ & The timestamp when layer l begins to calculate gradients. \\
% c & The non-overlapped communication cost in each iteration
\bottomrule
\end{tabular}
\label{tab:freq_notation}
\end{table}
